Foundation Models Knowledge Distillation For Battery Capacity Degradation Forecast

Accurate forecasting of lithium-ion battery capacity degradation is critical for reliable and safe operation, yet remains challenging under distribution shifts across scales and operating regimes. Here we investigate a time-series foundation model, that is, a large pre-trained time-series model for capacity degradation forecasting, and propose a degradation-aware fine-tuning strategy that aligns the model to capacity trajectories while retaining broadly transferable temporal structure. We instantiate this approach by fine-tuning the Timer model on 220,153 cycles of open-source charge-discharge records to obtain Battery-Timer. Using our released CycleLife-SJTUIE dataset, a real-world industrial collection from an energy-storage station with long-horizon cycling, we evaluate capacity generalization from small cells to large-scale storage systems and across varying operating conditions. Battery-Timer consistently outperforms specialized expert models. To address deployment cost, we further introduce knowledge distillation, a teacher-student transfer that compresses the foundation model's behavior into compact expert models. Distillation across several state-of-the-art time-series experts improves multi-condition capacity generalization while substantially reducing computational overhead, indicating a practical path to deployable cross-scale degradation forecasting by combining a foundation model with targeted distillation.

==> Sections/Information/Authors.tex <==


\author[1]{Joey Chan}[style=chinese,orcid=0009-0004-8100-1546]\ead{sjtu_chan_joey@sjtu.edu.cn}
%第几作者
%%通讯作者星标

%\credit{Methodology, Writing - Original Draft, Validation, Visualization}

\author[1]{Zhen Chen}[style=chinese,orcid=0000-0003-2590-0307]\ead{chenzhendr@sjtu.edu.cn}\cormark[1]

\ead[url]{https://me.sjtu.edu.cn/teacher_directory1/chenzhen.html}
%\credit{Conceptualization, Investigation, Resources, Supervision}

\author[1]{Ershun Pan}[style=chinese,orcid=0000-0001-6026-9755]\ead{pes@sjtu.edu.cn}
\ead[url]{https://ieem.sjtu.edu.cn/szdy/2953.html}
%第几作者
\affiliation[1]{organization={Department of Industrial Engineering and Management, School of Mechanical Engineering, Shanghai Jiao Tong University, Shanghai 200240, China}}
\cortext[1]{Corresponding author}
%\credit{Project administration, Writing - Review & Editing}

==> Sections/Information/Bibs.tex <==

\addcontentsline{toc}{section}{Reference}
\renewcommand\refname{Reference}
\begin{thebibliography}{99}
\bibitem{ref41} Omrani, M. M., & Jannesari, H. (2019). Economic and environmental assessment of reusing electric vehicle lithium-ion batteries for load leveling in the residential, industrial and photovoltaic power plants sectors. Renewable and Sustainable Energy Reviews, 116, 109413.
\bibitem{ref42} Wang, H., Li, Y. F., & Zhang, Y. (2023). Bioinspired spiking spatiotemporal attention framework for lithium-ion batteries state-of-health estimation. Renewable and Sustainable Energy Reviews, 188, 113728.
\bibitem{ref40} Vykhodtsev, A. V., Jang, D., Wang, Q., Rosehart, W., & Zareipour, H. (2022). A review of modelling approaches to characterize lithium-ion battery energy storage systems in techno-economic analyses of power systems. Renewable and Sustainable Energy Reviews, 166, 112584.
\bibitem{ref38} Meng, H., & Li, Y. F. (2019). A review on prognostics and health management (PHM) methods of lithium-ion batteries. Renewable and Sustainable Energy Reviews, 116, 109405.
\bibitem{ref34} Finegan, D. P., Zhu, J., Feng, X., Keyser, M., Ulmefors, M., Li, W. & Cooper, S. J. (2021). The application of data-driven methods and physics-based learning for improving battery safety. Joule, 5(2), 316-329.
\bibitem{ref35} Dey, S., Perez, H. E., & Moura, S. J. (2017). Model-based battery thermal fault diagnostics: Algorithms, analysis, and experiments. IEEE Transactions on Control Systems Technology, 27(2), 576-587.
\bibitem{ref36} Marcicki, J., Onori, S., & Rizzoni, G. (2010, January). Nonlinear fault detection and isolation for a lithium-ion battery management system. In Dynamic Systems and Control Conference (Vol. 44175, pp. 607-614).
\bibitem{ref37} Wei, J., Dong, G., & Chen, Z. (2019). Lyapunov-based thermal fault diagnosis of cylindrical lithium-ion batteries. IEEE Transactions on Industrial Electronics, 67(6), 4670-4679.
\bibitem{ref22} Li, Da & Zhang, Lei & Zhang, Zhaosheng & Liu, Peng & Deng, Junjun & Wang, Qiushi & Wang, Zhenpo. (2023). Battery safety issue detection in real-world electric vehicles by integrated modeling and voltage abnormality. Energy. 284. 128438. 10.1016/j.energy.2023.128438.
\bibitem{ref16} Cherdo, Y., Miramond, B., Pegatoquet, A., & Vallauri, A. (2023). Unsupervised Anomaly Detection for Cars CAN Sensors Time Series Using Small Recurrent and Convolutional Neural Networks. Sensors, 23(11), 5013. MDPI AG. Retrieved from http://dx.doi.org/10.3390/s23115013
\bibitem{ref39} Zhang, X., Liu, P., Lin, N., Zhang, Z., & Wang, Z. (2023). A novel battery abnormality detection method using interpretable Autoencoder. Applied Energy, 330, 120312.
\bibitem{ref17} A. R. Javed, M. Usman, S. U. Rehman, M. U. Khan and M. S. Haghighi, "Anomaly Detection in Automated Vehicles Using Multistage Attention-Based Convolutional Neural Network," in IEEE Transactions on Intelligent Transportation Systems, vol. 22, no. 7, pp. 4291-4300, July 2021, doi: 10.1109/TITS.2020.3025875.
\bibitem{ref5} Zhou, Y., Liang, X., Zhang, W., Zhang, L., & Song, X. (2021). VAE-based deep SVDD for anomaly detection. Neurocomputing, 453, 131-140.
\bibitem{ref6} Z. Ghrib, R. Jaziri and R. Romdhane, "Hybrid approach for Anomaly Detection in Time Series Data," 2020 International Joint Conference on Neural Networks (IJCNN), Glasgow, UK, 2020, pp. 1-7, doi: 10.1109/IJCNN48605.2020.9207013.
\bibitem{ref7} Ruff, L., Vandermeulen, R., Goernitz, N., Deecke, L., Siddiqui, S. A., Binder, A., Müller, E. & Kloft, M. (2018, July). Deep one-class classification. In International conference on machine learning (pp. 4393-4402). PMLR.
\bibitem{ref4} Kingma, D., Salimans, T., Poole, B., & Ho, J. (2021). Variational diffusion models. Advances in neural information processing systems, 34, 21696-21707.
\bibitem{ref18} Zhang, Junfeng & Zhang, Hui & Zhang, Xiaoxiong. (2021). Power Consumption Predicting and Anomaly Detection Based on Transformer and K-Means. Frontiers in Energy Research. 9. 779587. 10.3389/fenrg.2021.779587.
\bibitem{ref19} Y. Wang, N. Masoud and A. Khojandi, "Real-Time Sensor Anomaly Detection and Recovery in Connected Automated Vehicle Sensors," in IEEE Transactions on Intelligent Transportation Systems, vol. 22, no. 3, pp. 1411-1421, March 2021, doi: 10.1109/TITS.2020.2970295.
\bibitem{ref2} Chen, Y., Tian, Y., Pang, G., & Carneiro, G. (2022, June). Deep one-class classification via interpolated gaussian descriptor. In Proceedings of the AAAI Conference on Artificial Intelligence (Vol. 36, No. 1, pp. 383-392).
\bibitem{ref8} Akcay, S., Atapour-Abarghouei, A., & Breckon, T. P. (2019). Ganomaly: Semi-supervised anomaly detection via adversarial training. In Computer Vision–ACCV 2018: 14th Asian Conference on Computer Vision, Perth, Australia, December 2–6, 2018, Revised Selected Papers, Part III 14 (pp. 622-637). Springer International Publishing.
\bibitem{ref33} Xia, X., Pan, X., Li, N., He, X., Ma, L., Zhang, X., & Ding, N. (2022). GAN-based anomaly detection: A review. Neurocomputing, 493, 497-535.
\bibitem{ref9} Kingma, D. P., & Welling, M. (2013). Auto-encoding variational bayes. arXiv preprint arXiv:1312.6114.
\bibitem{ref24} Radford, A., Metz, L., Chintala, S.: Unsupervised Representation Learning with Deep Convolutional Generative Adversarial Networks. In: ICLR (2016)
\bibitem{ref25} Gregor, Karol, Danihelka, Ivo, Graves, Alex, and Wierstra, Daan. Draw: A recurrent neural network for image generation. arXiv preprint arXiv:1502.04623, 2015.
\bibitem{ref23} H. Hojjati and N. Armanfard, "DASVDD: Deep Autoencoding Support Vector Data Descriptor for Anomaly Detection," in IEEE Transactions on Knowledge and Data Engineering, doi: 10.1109/TKDE.2023.3328882.
\bibitem{ref26} Goldstein, M., & Dengel, A.R. (2012). Histogram-based Outlier Score (HBOS): A fast Unsupervised Anomaly Detection Algorithm.
\bibitem{ref27} T. R. Bandaragoda, K. M. Ting, D. Albrecht, F. T. Liu and J. R. Wells, "Efficient Anomaly Detection by Isolation Using Nearest Neighbour Ensemble," 2014 IEEE International Conference on Data Mining Workshop, Shenzhen, China, 2014, pp. 698-705, doi: 10.1109/ICDMW.2014.70.
\bibitem{ref28} Weglarczyk, Stanislaw. (2018). Kernel density estimation and its application. ITM Web of Conferences. 23. 00037. 10.1051/itmconf/20182300037.
\bibitem{ref29} Hubert, M, Debruyne, M, Rousseeuw, PJ. Minimum covariance determinant and extensions. WIREs Comput Stat. 2018;10:e1421. https://doi.org/10.1002/wics.1421
\bibitem{ref30} Breunig, M. M., Kriegel, H. P., Ng, R. T., & Sander, J. (2000, May). LOF: identifying density-based local outliers. In Proceedings of the 2000 ACM SIGMOD international conference on Management of data (pp. 93-104).
\bibitem{ref31} Dreiseitl S, Osl M, Scheibböck C, Binder M. Outlier Detection with One-Class SVMs: An Application to Melanoma Prognosis. AMIA Annu Symp Proc. 2010 Nov 13;2010:172-6. PMID: 21346963; PMCID: PMC3041295.
\bibitem{ref32} Kingma, D. P., & Welling, M. (2013). Auto-encoding variational bayes. arXiv preprint arXiv:1312.6114.
\end{thebibliography}

==> Sections/Tables/battery_timer.tex <==

\begin{table*}[htb]
    \renewcommand{\arraystretch}{1.2}
    \centering
    \caption{Comparison of Foundation Model Performance Before and After Fine-Tuning.}
    % \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{c|cccccccc}
        \Xhline{1.2pt}
       Condition &\multicolumn{8}{c}{\textbf{Capacity}} \\
        \hline
        Original Timer & \#1  & \#2  & \#3  & \#4 & \#5 & \#6 &\#7 & \#8 \\
        \hline
        RMSE   & 0.0778 & 0.1386 & 0.1217 &   0.0668       & 0.0598 & 0.0846 & 0.1033 & 0.1168 \\
        MAE   & 0.0685 & 0.1129  & 0.1122 &  0.0598       & 0.0532 & 0.0756  & 0.0924 & 0.1062 \\
        \Xhline{1.2pt}
        Battery Timer  & \#1  & \#2  & \#3  & \#4 & \#5 & \#6 &\#7 & \#8 \\
        \hline
        RMSE   & 0.0213 & 0.0894 & 0.0462 & 0.0937           & 0.0297 & 0.0236 & 0.0207 & 0.0208 \\
        MAE   & 0.0153 & 0.0689  & 0.0409 &  0.0627         & 0.0289 & 0.0204  & 0.0158 & 0.0176 \\
        \Xhline{1.2pt}
    \end{tabular}
    % }
    \label{battery_timer}
\end{table*}
